Semantically-Guided Representation Learning for Self-Supervised Monocular Depth

Self-supervised learning is showing great promise for monocular depth estimation, using geometry as the only source of supervision. Depth networks are indeed capable of learning representations that relate visual appearance to 3D properties by implicitly leveraging category-level patterns. In this work we investigate how to leverage more directly this semantic structure to guide geometric representation learning, while remaining in the self-supervised regime. Instead of using semantic labels and proxy losses in a multi-task approach, we propose a new architecture leveraging fixed pretrained semantic segmentation networks to guide self-supervised representation learning via pixel-adaptive convolutions. Furthermore, we propose a two-stage training process to overcome a common semantic bias on dynamic objects via resampling. Our method improves upon the state of the art for self-supervised monocular depth prediction over all pixels, fine-grained details, and per semantic categories.

==> extras/failure_cases.tex <==


\begin{figure}[t!]
	\centering
	\subfloat{\includegraphics[width=0.33\textwidth]{figures/failure/000000033_rgb.jpg}}
	\subfloat{\includegraphics[width=0.33\textwidth]{figures/failure/000000033_lab.png}}
	\subfloat{\includegraphics[width=0.33\textwidth]{figures/failure/000000033_vis2.jpg}}
	\\\vspace{-4mm}
	\subfloat{\includegraphics[width=0.33\textwidth]{figures/failure/000000140_rgb.jpg}} 
	\subfloat{\includegraphics[width=0.33\textwidth]{figures/failure/000000140_lab.png}}
	\subfloat{\includegraphics[width=0.33\textwidth]{figures/failure/000000140_vis2.jpg}}
	\caption{\textbf{Sensitivity of our proposed architecture} to inaccurate semantic segmentation predictions (black circles), and how it translates to inaccurate depth estimates. The left column shows the input RGB image, the middle column are the output predicted semantic classes, and the right column depicts the predicted semantically-guided depth maps.   
	}
	\label{fig:qualitative}
\end{figure}
